Percolation and Epidemic Processes in One-Dimensional Small-World Networks

We obtain tight thresholds for bond percolation on one-dimensional small-world graphs, and apply such results to obtain tight thresholds for the \emph{Independent Cascade} process and the \emph{Reed-Frost} process in such graphs. These are the first fully rigorous results establishing a phase transition for bond percolation and SIR epidemic processes in small-world graphs. Although one-dimensional small-world graphs are an idealized and unrealistic network model, a number of realistic qualitative epidemiological phenomena emerge from our analysis, including the epidemic spread through a sequence of local outbreaks, the danger posed by random connections, and the effect of super-spreader events.

==> trunk-full/Intro-old-2.tex <==

\section{New Introduction} \label{sec:newintro}

We should present the result according to the following approach:

\begin{itemize}
    \item Given a graph $G=(V,E)$ the bond percolation subgraph $G_p$  is the random graph obtained by    removing  each edge in  $E$ ...independently with prob $1-p$ where $p=p(e)$ is the bond percolation probability.... Bond percolation  has been widely studied in computer and network science since this processes  has clean connections with several aspects and applications of distributed systems: among them, we here remark its role as effective measures of the resiliency (fault-tolerance) of a network and, moreover, the fact that it is  equivalent to the  epidemic, information-spreading protocols, known as the Reed-Frost Model/Protocol...describe it...
    
    \item Typical   questions in this topic mainly concern the emergence of a giant connected component  and the  diameter of it,  and the related threshold phenomena. The latter typically depends on the specific considered class of graphs and on the edge probability $p$.
    
    \item Motivated by the study of epidemic protocols on networks, we here focus on   more   specific questions on    bond percolation. i) Given a fixed     (source) node how large is the size of the connected component in $G_p$ containing it? How does the subset of nodes within   distance $t$ from $s$ in $G_p$ grows as a function of $t$? Thanks to equivalence between bond percolation and RF model, it is easy to verify that the first question is equivalent to ask how many nodes, the source node will infect at the end of the epidemic protocol, while the second question refers to the   number of   nodes   that will be infected within time $t$. A further important question is to determine any geometrical  properties of the subset of infected nodes with respect to the metric introduced by the original graph $G$. To be more concrete, if, for instance, the original graph is the $d$-dimensional lattice, it is important to bound the infected area around the source as a function of time...
    
     It is clear that the above issues  are related to the typical  questions (i.e., size and   diameter of the giant connected component, and threshold phenomena). However, such quantities might turn to give only rough estimations of the questions we discussed above. For instance,  a linear lower bound on the diameter of the giant component does not necessarily exclude  that   many (e.g. $\Omega(n)$)   ''central'' nodes   might  have non negligible chances to infect a linear number of nodes in logarithmic time.
     
     \item   Just to get an initial idea of bond percolation, consider
       $G$  sampled from the    \Erdos\   graph distribution $\mathcal{G}_{n,q}$: then the distribution of
the percolation graph $G_p$, over the randomness of the generation of $G$ and
of the bond percolation process, is the same as the distribution of \Erdos\
random graphs $\mathcal{G}_{n,pq}$. Classical results from \Erdos\
random graph theory tell us that, for every $\epsilon >0$,  if $pqn < 1-\epsilon$, then all the connected components of
$\mathcal G_{n,pq}$ have, with high probability, size $\bigO_\epsilon (\log n)$ and there is no
large scale epidemic spreading; if $pqn > 1+\epsilon$ then there is, with high
probability, a giant component in $\mathcal G_{n,pq}$ of size $\Omega_\epsilon (n)$ and
epidemic spreading affects on average a constant fraction of nodes within logarithmic time. That is, we see a threshold behavior at $pnq = 1$, i.e., at the point at which $p\bar d =1$, where $\bar d = qn$ is the average degree of $G$.
In other graphs, however, the critical value for $p \bar d$ is not 1.  In a
cycle, for example, if $p< 1-\epsilon$ then every connected component has size
$\bigO_\epsilon (\log n)$, and there is no large-scale spreading; if $p=1$ then
$G_p$ is connected and all nodes are reached by the disease. This means that,
in a cycle, the critical value of $r_0$ that determines if large-scale
contagion takes place is 2, rather than 1.


     
     
     \item In this paper we are interested in network models that are simple enough to
admit an analytical study but complex enough to exhibit phenomena such as the
presence of outbreaks and the distinction between local and
non-local connections. We are interested in studying bond percolation in the simplest families of
graphs that exhibit a distinction between ``local'' and
``long-distance'' connections, that is, a model similar to the Watts-Strogatz
model of ``small-world'' graphs, $\SWGm$ for short,  in which we have a cycle
(representing the local connections) augmented with random edges, which we call
{\em bridges}. 

Our analysis covers many well-studied  versions of 1-dimensional small world graphs proposed in the literature \cite{}: such versions essentially depend on the specific  random  distribution the  bridges are  generated.
In detail, we consider  two main classes: (i)  erods renij  random uniform      distributions \cite{}, 
where  each pair of node has the same chance to be connected by a bridge; (ii)
regular random graphs....
 

\item As for   the first class of  models.....describe shortly the most interesting results

\item As for the second class of models...describe shortly the most interesting results


\item Describe the structure of this paper

   
   
   
    
    
\end{itemize}

\section{Our Results  } \label{sec:ourresults}
%We study      Watts-Strogatz models $\SWGm$ where the graphs $G=(V, E_1 \cup E_2)$  where  $E_1$ is a cycle (representing the local connections) and $E_2$ is the subset of    random edges, which we call {\em bridges}.   As for the latter, we consider the    two alternatives:

 We study two different but similar models for a small-world network $G=(V,E)$, inspired by the popular Watts-Strogatz model \cite{}.  In both the considered models, the set of edges $E$ is the union of a deterministic cycle $E_1$ (representing the local connections) and a set $E_2$ of random edges, which we call \textit{bridges}.    As for the latter, we consider the    two alternatives for the distribution of $E_2$
 which define two different models for the small-world network, described in the following definitions.

\begin{definition}[$1$-Dimensional Small-World Graphs - \SWG ]\label{def:small-world}
For every  $n \geq 3$ and $0 \leq q \leq 1$, the distribution \SWG\ is sampled
by generating a one-dimensional small-world graph $G=(V,E)$, where $|V|=n$, $E
= E_1 \cup E_2$, $(V,E_1)$ is a cycle, and $E_2$ is the set of random edges of
an \Erdos\ random graph ${\mathcal G}_{n,q}$, in which edges are sampled
independently, and each pair of nodes has probability $q$ of being an edge.
\end{definition}

%The above small-world graph model generates sparse graphs with unbounded
%degree. The maximum  degree of a graph sampled from $\SWGm(n,1/n)$, like the
%maximum degree of a ${\mathcal G}_{n,1/n}$ random graph, is on average
%$\Theta(\log n/\log\log n)$.
The above small-world graph, when $q=1/n$, generates a sparse graphs with unbounded degree. Indeed, the maximum degree of an \Erdos \ random graph $\mathcal{G}_{n,1}$ is on average $\Theta(\log n / \log \log n)$. Instead, the following model generates a bounded-degree graphs.

\begin{definition}[$3$-regular $1$-Dimensional  Small-World Graphs - \SWGreg ]\label{def:small-world-3reg}
For every  even $n \geq 4$, the distribution  \SWGreg\ is sampled by generating
a one-dimensional small-world graph  $G=(V, E)$, where $|V|=n$, $E = E_1 \cup
E_2$, $(V,E_1)$ is a cycle, and $E_2$ is the set of edges of a uniformly chosen
perfect matching on $V$.
\end{definition}

We observe that the each node in the above small-world graph $G$ has always degree bounded by $3$\footnote{If we let $G$ to be a multigraph, then the graph is 3-regular.}.

%\begin{itemize} 

%\item The subset $E_2$ of bridges   form a random perfect matching over the nodes of the
%cycle (this will assume that the number  $n$ of nodes is even), giving rise to
%a graph of maximum degree 3.
%We denote the resulting distribution of graphs as \SWGreg;

%\item  The  bridges in   $E_2$ are  selected as in an \Erdos\ random graph
%$\mathcal{G}_{n,q}$. We denote the resulting distribution of graphs as \SWG. We
%will consider the case $q=c/n$ for any fixed constant $c > 0$, noticing that
%the case $c=1$ yields a number of  bridge edges that is concentrated around
%$n/2$, similarly to the first case. 

%\end{itemize}

Our main results are to establish sharp thresholds for the critical percolation probability $p$ in both
models. In particular, we are interested in fully rigorous analysis, avoiding mean-field
approximations or approximations that treat certain  correlated events as independent, which are common in the analysis of complex networks in
the physics literature. While such approximations are necessary when dealing
with otherwise intractable problems, they can fail to capture subtle
differences between models. For example, for $q = 1/n$, the marginal distributions of 
bridge edges are the same in the two models above, while correlations between edges are non-existing in the \SWG\ model
and very small in the \SWGreg model. Yet, though the two models have similar
expected behaviors and are good approximations of each other, our rigorous
analysis shows that the two models exhibit notably different thresholds.

%Our main results are to establish sharp thresholds for the critical percolation probability $p$ in both

According to our interest on the epidemic interpretations of bond percolation discussed in the Introduction, we  here state  our results in terms of:  ``\emph{how many nodes are reachable  from a given source subset and in how many hops}''.  

\begin{theorem}[Percolation on the \SWG model] \label{thm:gen_overthershold}
Let $V$ be a set of $n$ vertices, $I_0 \subseteq V$, and $p>0$ be a bond percolation  probability. For any constant
$c>0$,  sample a graph $G=(V, E_1 \cup E_2)$ from the $\SWGm(n,c/n)$ distribution, and consider the percolation subgraph $G_p$.

\begin{enumerate}
\item  Let $p > \frac{\sqrt{c^{2} + 6c +1}-c-1}{2c} + \varepsilon$. Then, with
probability $\Omega_\varepsilon(1)$, there are $\Omega_\varepsilon(n)$ nodes within distance $\bigO(\log n)$ from $I_0$, even if $|I_0| = 1$. 



\iffalse 
a constant $\gamma_\varepsilon$ exists such that,  for every   $t \leq \gamma_\varepsilon \log n$,  the number of  nodes at distance at most $t$ from $I_0$ in $G_p$ are at least  $|I_0|(1+\Omega_\varepsilon(1))^t$, and, moreover,   this number becomes  $\Omega_\varepsilon(n)$,  for some $t = \bigO_\varepsilon(\log n)$, even if $|I_0| = 1$.



\andy{NO: c'e' una fase di bootstrap in cui la crescita e' dimostrata essere solo lineare e non esponenziale....}
\fi 


\item Let $p > \frac{\sqrt{c^{2} + 6c +1}-c-1}{2c} + \varepsilon$ and 
$|I_0|\geq\beta_\varepsilon\log n$ for a sufficiently large constant
$\beta_\varepsilon$ (that depends on $\varepsilon$ but not on $n$).
Then, \emph{with high  probability}\footnote{As usual, we say that an event
$\mathcal{E}_n$ occurs \emph{with high probability} if $\Prc{ \mathcal{E}_n}
\geq 1-(1/n)^{\Omega(1)}$. } (for short, \emph{w.h.p.}), 
%a constant $\gamma_\varepsilon$ exists such that,  for every   $t \leq \gamma_\varepsilon \log n$, 
the number of  nodes at distance at most $t$ from $I_0$  grows exponentially in $t$,  reaching magnitude  $\Omega_\varepsilon(n)$,  for some $t = \bigO_\varepsilon(\log n)$;
    
\item if $p<\frac{\sqrt{c^{2} + 6c +1}-c-1}{2c} - \varepsilon$, then, w.h.p.,
 the total
number of  nodes connected to $I_0$ in $G_p$ is $O_\varepsilon(|I_0|\log n)$.
\end{enumerate}
\end{theorem}


Some remarks are in order. In the theorem above, probabilities are taken
both over the randomness in the generation of the graph $G$ and over the
randomness of the percolation process. The lower bounds in claims 1 and 2 of
the theorem are proved by studying a BFS-like visit of the graph; we first
establish a more general form of claim 2, by showing that once the visit has
at least $\beta_\varepsilon \log n$ nodes in the queue, it has a high probability
of finding $\Omega_\varepsilon (n)$ nodes within distance $\bigO_\varepsilon (\log
n)$ from the nodes visited up to that point; to prove claim 1 we then 
show that there is at least constant probability that in the first
$\bigO_\varepsilon (\log n)$ steps of the visit the queue grows to a size at least
$\beta_\varepsilon \log n$. We provide more details of our techniques in
Section~\ref{sec:Proof Ideas}, while here we observe a direct consequence of the above theorem and its proof.

\begin{cor}[Percolation on the \SWG model] Under the hypothesis of Theorem \ref{thm:gen_overthershold}, if $p>\frac{\sqrt{c^{2} + 6c +1}-c-1}{2c} + \varepsilon$,  then, w.h.p.,
      a subset of nodes of size $\Omega_\varepsilon(n)$ exists 
      that induces   a   subgraph  of $G_p$ having  diameter $\bigO(\log n)$. While, if  $p<\frac{\sqrt{c^{2} + 6c +1}-c-1}{2c} - \varepsilon$, then, w.h.p., $G_p$ is formed by connected components of size $\bigO(\log n)$.
\end{cor}










Finally, we highlight the sharp result
given by the theorem on the $\SWGm(n,c/n)$ model for the case $c = 1$:
similarly to the regular \SWGreg model, each node here has about one bridge
edge in average, and the obtained critical value for the percolation probability
$p$ turns out to be $\sqrt{2}-1$. An analysis of the critical value for
the \SWGreg model is given by the next two results, while a detailed comparison of the two
models is provided after Theorem~\ref{th:reg.upper} below.


\begin{theorem}[Percolation on the  \SWGreg model]\label{thm:main_matching}
Let $V$ be a set of $n$ vertices, $I_0 \subseteq V$, and $p>0$ be a bond percolation  probability. Sample a graph $G=(V, E_1 \cup E_2)$ from the \SWGreg distribution,  and consider the percolation subgraph $G_p$:

\begin{enumerate}
\item if $p>1/2+\varepsilon$, then with probability $\Omega_\varepsilon(1)$,
there are  $\Omega_\varepsilon(n)$ connected to $I_0$ in $G_p$;

\item Let $p>1/2+\varepsilon$ and  $|I_0|\geq\beta_\varepsilon\log n$ for a sufficiently large constant $\beta_\varepsilon$ (that depends on $\varepsilon$ but not on $n$). Then w.h.p., there are  $\Omega_\varepsilon(n)$ connected to $I_0$ in $G_p$;

\item if $p<1/2-\varepsilon$, then, w.h.p.,  the total number of  nodes connected to $I_0$ in $G_p$ is $O_\varepsilon(|I_0|\log n)$.
\end{enumerate}
\end{theorem}

In the above theorem, the first two  statements hold with constant probability over
the randomness of the generation of $G$ and the randomness of the contagion
process. 

The third statement holds with probability $1$ over the randomness of $G$ and
\emph{with high probability} over the randomness of the contagion process, and
it is a special case of the following more general result of ours.

\begin{theorem}[Percolation on bounded-degree graphs] 
\label{th:reg.upper}
Let $G=(V,E)$ be a graph of maximum degree $d$, $\varepsilon >0$ be an
arbitrary positive number, $p < (1-\varepsilon)/(d-1)$  be a bond percolation  probability, and $I_0$ be a subset of $V$.  
  Consider the percolation subgraph $G_p$.  Then,
w.h.p.,   the number of nodes connected to $I_0$ in $G_p$
is  $\bigO_\varepsilon ( |I_0| \log n)$.
\end{theorem}




\subsection{Consequences of our results for epidemic models}
As remarked in Section \ref{sec:newintro}, bond percolation is equivalent to the popular (SIR) RF epidemic model: roughly speaking, the nodes at distance $t$ in $G_p$ from the source nodes are exactly those that will get the infection at time $t$ according to the  RF protocol.
Then, in terms of epidemic processes, our results have the following interesting consequences.

Because of a mix of local and random edges, epidemic spreading in the above
models proceeds as a sequence of outbreaks, a process that is made explicit in
our rigorous analysis, where we see the emergence of two qualitative
phenomena that are present in real-world epidemic spreading. 

One is that the presence of long-distance random connections has a stronger
effect on epidemic spreading than local connections, motivating lockdown
measures that shut down long-distance connections.  This can be seen,
quantitatively, in the fact that the critical probability in a cycle is $p =
1$, corresponding to a critical $r_0$ equal to 2. On the other hand, the
presence of random matching edges or random $\mathcal{G}_{n,c/n}$ edges in the
setting $c = 1$ defines networks in which the critical $r_0$ is, respectively,
$1.5$ and $3\cdot (\sqrt 2 -1) \approx 1.24$, meaning that notably fewer local
infections can lead to large-scale contagion on a global scale.

The other phenomenon is that  the irregular networks of the $\SWGm(n,c/n)$
model in the case $c=1$ show a significantly lower critical probability, i.e.
$\sqrt 2 -1 \approx .41$, than the  critical value $.5$ of the nearly regular networks of
the \SWGreg model, though they have the same number of edges (up to lower order
terms) and very similar distributions. As a further evidence of this
phenomenon, we remark the scenario yielded by the random irregular networks
sampled from the $\SWGm(n,c/n)$ distribution with $c$ even smaller than $1$:
for instance, the setting $c = .7$, though yielding a much sparser topology
than the \SWGreg networks, has a critical probability which is still smaller
than $.5$. Moreover, this significant difference between the $\SWGm(n,c/n)$
model and the regular $\SWGm$ one holds even for more dense regimes. In detail,
Theorem~\ref{th:reg.upper} implies that the  almost-regular version of $\SWGm$
in which $c$ independent random matchings are added to the ring of $n$ nodes
has a critical probability at least $1/(c+1)$. Then, simple calculus shows that
the critical probability given by Theorem~\ref{thm:gen_overthershold} for the
$\SWGm(n,c/n)$ model is smaller than $1/(c+1)$, for any choice  of the
density parameter $c$.

The most significant difference between the two distributions above  is the
presence of a small number of high-degree vertices in $\SWGm(n,c/n)$,
suggesting that even a small number of ``super-spreader'' nodes can have major
global consequences.


\subsection{Extensions of our results for epidemic models}

\paragraph{Longer node activity and incubation.}
Natural generalizations of the setting considered in this work include models in which i) the interval of time
during which a node is infectious (i.e., the \emph{activity period}) follows some (possibly node-dependent) distribution and/or ii) once infected, a node only becomes infectious after an \emph{incubation} period, whose duration again follows some distribution.
While the introduction of activity periods following general distributions may considerably complicate the analysis, our approach rather straightforwardly extends to
two interesting cases, in which the incubation period of each node is a random variable (as long as incubation periods are independent) and/or the activity period of a node consists of $k$
consecutive units of time, with $k$ a fixed constant. 
This generalized model with random, node-dependent incubation periods corresponds to a discrete,
synchronous version of the $\mathrm{SEIR}$ model,\footnote{With respect to \SIR, for each node we have a fourth, \emph{Exposed} state, corresponding to the incubation period of a node.} which 
was recently considered as a model of the COVID-19 outbreak in Wuhan \cite{lin2020conceptual}.
These extensions are formalized and discussed in Appendix \ref{sec:further}.

\paragraph{Non-homogenous contagion probability.}





\section{Related Works} \label{sec:related_new}

\andy{TO BE UPDATED}

As far as we know, our results are the first rigorous ones to establish
threshold phenomena in small-world graphs for the \SIR\ process  and for the
bond percolation process.

There has been some previous work on studying sufficient conditions for the
\SIR\ process  to reach a sublinear number of vertices. 

 
In~\cite{DGM06}, for a symmetric, connected graph $G = (V,E)$, Draief et al
prove a general lower bound on the critical point in the Independent Cascade
model in terms of spectral properties. Further versions of such bounds for
special cases have been subsequently derived in~\cite{LKAK16,LSV14}.
Specifically, if one lets $P$ be the matrix such that $P(u,v) = p(u,v)$ is the
probability of the edge $\{u,v\}$, and $P(u,v) = 0$ if $\{u,v\}\not\in E$, and
if one call $\lambda$ the largest eigenvalue of $P$, then $\lambda <
1-\epsilon$ implies that for a random start vertex $s$ we have that the
expected number of vertices to which $s$ spreads the infection is $o_\epsilon
(n)$.

In the special case in which all probabilities are the same, $P = p \cdot A$,
where $A$ is the adjacency matrix of $G$, and so the condition is asking for $p
< (1-\epsilon)/ \lambda_{\max{}} (A)$.

This condition is typically not tight, and it is never tight in the
``small-worlds'' graphs   we consider:

\begin{itemize}

\item In the  \SWGreg model, the largest eigenvalue of the adjacency matrix is
$3-o(1)$, but the critical probability is $1/2$ and not $1/3$;

\item In the $\SWGm(n,1/n)$ model of a cycle plus \Erdos\ edges, the largest
eigenvalue of the adjacency matrix is typically $\Omega(\sqrt{ \log n /
\log\log n})$, because we expect to see vertices of degree $\Omega(\log n /
\log\log n)$ and the largest eigenvalue of the adjacency matrix of a graph is
at least the square root of its maximal  degree. The spectral bound would only
tell us that the infection dies out if $p = \bigO(\sqrt{\log\log n / \log n})$,
which goes to zero with $n$.  A better way to use the spectral approach is to
model together the randomness of the small-world graph and the randomness of
the percolation; in this case we have matrix $P(u,v)$ such that $P(u,v)=p$ for
edges of the cycle and $P(u,v) = p/n$ for the other edges. This matrix has
largest eigenvalue $3p-o(1)$ and so the spectral method would give a
probability of $1/3$, while we are able to locate the threshold at $\sqrt 2
-1\approx .41$.
\end{itemize}

In any family of $d$-regular graphs, the largest eigenvalue of the adjacency
matrix is $d$, and so the spectral bound gives that the critical threshold is
at least $1/d$; our Theorem~\ref{th:reg.upper} shows the stronger bound that
the critical threshold is at least $1/(d-1)$.

We are not aware of previous rigorous results that provide sufficient
conditions for the Independent Cascade process to reach $\Omega(n)$ nodes
(either on average or with high probability) in general graphs, or for the
equivalent question of proving that the percolation graph of a given graph has
a connected component with $\Omega(n)$ vertices.


%\andy{Cambiare qui sotto: la discussione della nostra analisi e' ora sopra}

Our analysis, as discussed in the previous subsection, proceeds by analysing a
BFS-like visit of the percolation graph. This is also the way in which large
components in the percolation of infinite trees and in random graphs have been
studied before, but this idea requires considerable elaboration to work in our
setting, given the mix of fixed edges and random edges in the small-world
model, and the complicated dependencies on the past history that one has to
control in the analysis of the visit.





More generally, there is a very large body of work devoted to study of models of epidemic
spreading, as surveyed in~\cite{VespietAl15,Wang_2017}. In the following, we
review analytical studies of Independent Cascade on finite graphs.

In the Computer Science community, to the best of our knowledge, Kempe et al~\cite{KKT15}
were the first to investigate this model in an optimization perspective, in the context
of viral marketing and opinion diffusion. In particular, they introduced the \emph{Influence
Maximization} problem, where the goal is to find a subset of $k$ nodes of an underlying graph
to infect at time $t = 0$, so as to maximize the expected number of infected
nodes at the end of the Independent Cascade process. They prove this is an
$NP$-hard problem and show a polynomial time   algorithm achieving  constant
approximation.  Further approximation results on  a version of \emph{Influence
Maximization} in which the infection time is considered can be found
in~\cite{CWZ12,LGD12}.

A fundamental and rigorous study of bond percolation in random graphs has been proposed by Bollob\'as et al in~\cite{Bollo07}. 
They establish a coupling
between the bond percolation process and a suitably defined branching process.
In the   general class of inhomogenous \Erdos\ random graphs, calling $Q = \{
q_{u,v}\}$   the edge-probability matrix,  they derived the critical point
(threshold) of the phase transition and  the size of the giant component above
the transition. The  class  of inhomogeneous random graphs to which their
analysis applies includes  generative models that have been studied in the
complex network literature. For instance, a version of the Dubin's
model~\cite{Durrett1990ATT} can be expressed in this way, and so can the
\emph{mean-field scale-free model}~\cite{Bollobs2004TheDO}, which is, in turn,
related to the   Barabási–Albert model~\cite{Barab509}, having the same
individual edge probabilities, but with edges present independently. Finally,
we observe that the popular CHKNS model introduced by  Callaway et
al~\cite{CDHKNS01} can be analyzed using an edge-independent version of this
model. Indeed, they consider a random graph-formation process where, after
adding each node,   a Poisson  number of edges is added to the graph, again
choosing the endpoints of these edges uniformly at random.  For all such
important classes of random graph models, they show tight bounds for the
critical points and the relative size of the giant component beyond the phase
transition.

In our setting, if we sample a graph from $\SWGm(n,q)$ and then consider the
percolation graph $G_p$, the distribution of $G_p$ is that of an inhomogenous
\Erdos\ graph in which the cycle edges have probability $p$ and the remaining
edges have probability $pq$ (the \SWGreg model, however, cannot be expressed as
an inhomogenous \Erdos\ graph).

Unfortunately, if we try to apply the results of~\cite{Bollo07} to the
inhomogenous random graph equivalent to percolation with parameter $p$ in the
$\SWGm(n,q)$ model, we do not obtain tractable conditions on the critical
value $p$ for which the corresponding graph has a large connected component of
small diameter, which is the kind of result that we are interested in proving.



Bond percolation and the  \SIR process on the class of $1$-dimensional small-world networks (that is,
graphs obtained as the union of a cycle and of randomly chosen edges) have been
studied in~\cite{MCN00}: using numerical approximations on the moment
generating function, non-rigorous bounds on the critical threshold    have been
derived while analytical results are given neither  for the expected size of
the number of infected nodes above the transition phase of the SIR process nor
for the infection time.  Further non-rigorous results on the critical points of
several classes of complex networks have been derived in~\cite{LRSV14,LKAK16}
(for good surveys see~\cite{VespietAl15,Wang_2017}).


In \cite{BB01,Bis04,Bis11}, different versions of the bond percolation process has been studied in 
small-world structures formed by a $d$-dimensional grid augmented by random edges that follow a power-law distribution: a bridge between points $x$ and $y$ is selected with probability $\sim 1/\dist(x,y)^{\alpha}$, where $d(x,y)$ is the grid distance between $x$ and $y$ and $\alpha$ is a fixed  power-law parameter. Beside other aspects, each version is  characterized by: (1)  whether the grid is infinite or finite, and  (2) whether the grid edges (local ties) do percolate with probability $p$  or not. 
Research in this setting has focused  on the  emergence of a large connected component and on  its diameter as functions of the parameters $d$ and $\alpha$, while, to the best of our knowledge,  no rigorous threshold bounds are known for the contagion probability $p$. Interestingly enough, in both power-law  infinite and finite structures (i.e. graphs), such studies globally show three different regimes of behaviour depending on the range the parameter $\alpha$ belongs to w.r.t. the dimension $d$. 




%%%%%%%%%%%% Proofs Ideas (Part I)
\input{./trunk-full/proofs_ideas_part_1.tex}
%%%%%%%%%%%%





==> trunk-full/Intro-old.tex <==



\section{Old Introduction} \label{sec:intro}

We are interested in {\em SIR models} of epidemic spreading of infectious
diseases. In such models, at any given time, each individual of the population
is in one of three possible states: a {\em susceptible state}, which is that of
individuals who have never come in contact with the disease; an {\em
infectious} state, which is that of individuals who have been infected and have
an active form of the disease, which they can spread; and a {\em recovered}
state, which is that of individuals who have been infected in the past and are
now recovered and immune.

In a \SIR model, infectious individuals may spread the disease to susceptible
individuals that they come in contact with. In the simplest version of these
models, called \emph{homogeneous}, or
\emph{fully-mixed}~\cite{CWLC13,VespietAl15}, each infectious individual has
the ability to spread the disease to an average of $r_0$ random individuals,
provided that they are susceptible. If a fraction $\sigma$ of the population is
susceptible at a given time, then each infectious individual spreads the
disease on average to $\sigma r_0$ other people.  In this framework, if $r_0
<1$, the number of infectious individuals tends to decrease exponentially with
time, and goes to zero; if $r_0 > 1$, the number of infectious individuals
grows exponentially at first, then, after the total number of recovered and
infectious individuals goes above a fraction $1-1/r_0$ of the population (the
{\em herd immunity} threshold), the number of infectious individuals decreases
and goes to zero.

In {\em network} models of SIR epidemic spreading, we have a graph $G = (V,E)$
whose vertices represent the individuals in the population, and edges $(u,v)
\in E$ represent the event that $u$ and $v$ come into contact and that, if $u$
is infectious and $v$ is susceptible, it is possible for $u$ to infect $v$ (and
vice versa). 

Network models are able to express features of epidemic spreading that are not
captured by more basic SIR models, such as the fact that the spread of the
disease proceeds by a sequence of {\em outbreaks}, which take place when a
person all whose close contacts are susceptible comes into random contact with
an infectious individual (by dining in a restaurant, or going to a concert, or
taking public transit, or traveling to a different place). If the underlying
graph has a distinction between ``local edges'' connecting people that live
together or that have other kinds of frequent contact, and ``long-distance
edges'' representing other forms of random contact with strangers, it is
possible to model the effect of lockdown measures that shut down 
``long-distance'' connections, an effect that is not representable in more
basic models.

To have a fully defined network model, we have to specify the underlying graph
(or possibly a family of time-varying graphs), and we have to specify, for each
edge $\{ u,v \}$, the probability $p(u,v)$ that if $u$ is infectious and $v$ is
susceptible we have the event that $u$ spreads the disease to $v$. Furthermore,
we have to specify the (distribution of the) of the time during which each
infectious node stays infectious before recovering. This usually leads to
complex models, that have a large number of tunable parameters, and that are more suitable to an experimental than to an
analytical study. 

In this paper we are interested in network models that are simple enough to
admit an analytical study but complex enough to exhibit phenomena such as the
presence of outbreaks and the distinction between local and
non-local connections.

 

In the well-studied {\em Independent Cascade} model \cite{KKT15,CWLC13},
one assumes that each infectious node stays infectious for a fixed duration of one unit of time, with
all infections happening also at discrete time steps. 
Epidemic spreading in the Independent Cascade model has been analyzed both in the setting of epidemiology, as
a model of literal disease spreading,  and as a model of the ``viral''
spreading of ideas, opinions and memes. In this last setting, the Independent Cascade model has
also been considered in an optimization perspective, as we discuss in more detail in Section \ref{subse:related}.


The {\em Reed-Frost}
model is the restriction of the Independent Cascade model to the case in which
all edge  probabilities are equal to a single parameter $p$ which, in this
paper, we call \emph{infection} or \emph{contagion} probability.
We refer the reader to \cite{DGM06,LKAK16} for an overview of these models,
while in the following, when we refer to a
{\em SIR} infection process on a network, we will always mean the Reed-Frost
model, unless otherwise specified.


In the Independent Cascade model on a graph $G = (V,E)$, the analog of $r_0$,
i.e. the average number of nodes that a random infectious node can spread the
disease to, is $\frac 1 {|V|} \sum_{u \in V} \sum_{\{ u,v\} \in E} p(u,v)$
which, in the Reed-Frost model, simplifies to $p \bar d$, where $\bar d=
2|E|/|V|$ is the average degree of $G$.

Providing an analytical study of the Reed-Frost model in a family of graphs is equivalent to answering clean questions about
bond percolation in that family of graphs. {\em Bond Percolation} in a graph $G$ refers to the
study of the number of nodes reachable from a start node $s$ in the percolation
random graph $G_p$ obtained from $G$ by removing  each edge, independently,
with probability $1-p$ and keeping it with probability $p$.

In particular (see the results of~\cite{KKT15} which we recall in Theorem
\ref{thm:equivalence} below) if $G$ is a graph, $p$ is an infection probability
along edges, and $I_0$ is a set of initially infectious nodes, then the
distribution of nodes that are infectious after $t$ steps in the Reed-Frost
model is precisely the distribution of nodes that are at distance $t$ from
$I_0$ in the percolation graph $G_p$. Similarly, the distribution of nodes that
are recovered after $t$ steps is precisely the distribution of nodes that are
at distance $< t$ from $I_0$ in $G_p$.

\iffalse
For example, if $G$ is a clique on $n$ vertices, we get back the fully mixed
SIR model with $r_0 = pn$, and the percolation graph $G_p$ is distributed like
an \Erdos\ random graph $\mathcal{G}_{n,p}$. The classical results from \Erdos\
random graph theory are in accord with the fundamental results about the fully
mixed SIR model: if $pn < 1-\epsilon$, then all the connected components of
$G_p$ have, with high probability, size $\bigO_\epsilon (\log n)$ and there is no
large scale epidemic spreading; if $pn > 1+\epsilon$ then there is, with high
probability, a giant component in $G_p$ of size $\Omega_\epsilon (n)$ and
epidemic spreading affects on average a constant fraction of nodes.

\fi 




For example, if $G$ is an \Erdos\ random graph $\mathcal{G}_{n,q}$ then the distribution of
the percolation graph $G_p$, over the randomness of the generation of $G$ and
of the bond percolation process, is the same as the distribution of \Erdos\
random graphs $\mathcal{G}_{n,pq}$. Classical results from \Erdos\
random graph theory tell us that, for every $\epsilon >0$,  if $pqn < 1-\epsilon$, then all the connected components of
$\mathcal G_{n,pq}$ have, with high probability, size $\bigO_\epsilon (\log n)$ and there is no
large scale epidemic spreading; if $pqn > 1+\epsilon$ then there is, with high
probability, a giant component in $\mathcal G_{n,pq}$ of size $\Omega_\epsilon (n)$ and
epidemic spreading affects on average a constant fraction of nodes. That is, we see a threshold behavior at $pnq = 1$, i.e., at the point at which $p\bar d =1$ (i.e., the point at which the parameter $r_0$ is 1), where $\bar d = qn$ is the average degree of $G$, in agreement with the fully mixed SIR model.


In other graphs, however, the critical value for $p \bar d$ is not 1.  In a
cycle, for example, if $p< 1-\epsilon$ then every connected component has size
$\bigO_\epsilon (\log n)$, and there is no large-scale spreading; if $p=1$ then
$G_p$ is connected and all nodes are reached by the disease. This means that,
in a cycle, the critical value of $r_0$ that determines if large-scale
contagion takes place is 2, rather than 1.



\subsection{Our results}
We are interested in studying the Reed-Frost model in the simplest families of
graphs that exhibit a distinction between ``local'' and
``long-distance'' connections, that is, a model similar to the Watts-Strogatz
model of ``small-world'' graphs, $\SWGm$ for short,  in which we have a cycle
(representing the local connections) augmented with random edges, which we call
{\em bridge} edges. 

We consider two alternatives for  random bridge edges:
\begin{itemize} 
\item Bridge edges form a random perfect matching over the nodes of the
cycle (this will assume that the number  $n$ of nodes is even), giving rise to
a graph of maximum degree 3.\footnote{If the edges of the random perfect
matching are disjoint from the edges of the cycle, then the graph is 3-regular.}
We denote the resulting distribution of graphs as \SWGreg;
\item  Bridge edges are selected as in an \Erdos\ random graph
$\mathcal{G}_{n,q}$. We denote the resulting distribution of graphs as \SWG. We
will consider the case $q=c/n$ for any fixed constant $c > 0$, noticing that
the case $c=1$ yields a number of  bridge edges that is concentrated around
$n/2$, similarly to the first case. 
\end{itemize}

We are interested in fully rigorous analysis, avoiding mean-field
approximations or approximations that treat certain  correlated events as independent, which are common in the analysis of complex networks in
the physics literature. While such approximations are necessary when dealing
with otherwise intractable problems, they can fail to capture subtle
differences between models. For example, for $c = 1$, the marginal distributions of 
bridge edges are the same in the two models above, while correlations between edges are non-existing in the \SWG\ model
and very small in the \SWGreg model. Yet, though the two models have similar
expected behaviors and are good approximations of each other, our rigorous
analysis shows that the two models exhibit notably different thresholds.

Our main results are to establish sharp thresholds for the critical contagion probability $p$ in both
models.


\begin{theorem}[\SIR on the \SWG model] \label{thm:gen_overthershold-old}
Let $V$ be a set of $n$ vertices, $I_0 \subseteq V$, and $p>0$ be a contagion probability. For any constant
$c>0$,  sample a graph $G = (V,E)$ from the $\SWGm(n,c/n)$ distribution, and
run the Reed-Frost \SIR\ process on $G$ with contagion probability $p$ and with
the vertices in $I_0$ infectious at time 0. Then:

\begin{enumerate}
\item If $p>\frac{\sqrt{c^{2} + 6c +1}-c-1}{2c} + \varepsilon$,  then, with
probability $\Omega_\varepsilon(1)$, the \SIR \ process infects
$\Omega_\varepsilon(n)$ nodes within time $\bigO_\varepsilon(\log n)$, even if
$|I_0| = 1$;

\item if $p > \frac{\sqrt{c^{2} + 6c +1}-c-1}{2c} + \varepsilon$ and
$|I_0|\geq\beta_\varepsilon\log n$ for a sufficiently large constant
$\beta_\varepsilon$ (that depends on $\varepsilon$ but not on $n$), then,
\emph{with high  probability}\footnote{As usual, we say that an event
$\mathcal{E}_n$ occurs \emph{with high probability} if $\Prc{ \mathcal{E}_n}
\geq 1-(1/n)^{\Omega(1)}$. } (for short, \emph{w.h.p.}),  the \SIR \ process
infects $\Omega_\varepsilon(n)$ nodes within time $O_\varepsilon(\log n)$;
    
\item if $p<\frac{\sqrt{c^{2} + 6c +1}-c-1}{2c} - \varepsilon$, then, w.h.p.,
the \SIR \ process stops within $O_\varepsilon(\log n)$ rounds and the total
number of infectious nodes is $O_\varepsilon(|I_0|\log n)$.
\end{enumerate}
\end{theorem}

Some remarks are in order. In the theorem above, probabilities are taken
both over the randomness in the generation of the graph $G$ and over the
randomness of the infection process. The lower bounds in parts (1) and (2) of
the theorem are proved by studying a BFS-like visit of the graph; we first
establish a more general form of part (2), by showing that once the visit has
at least $\beta_\epsilon \log n$ nodes in the queue, it has a high probability
of finding $\Omega_\epsilon (n)$ nodes within distance $\bigO_\epsilon (\log
n)$ from the nodes visited up to that point; to prove part (1) we then 
show that there is at least constant probability that in the first
$\bigO_\epsilon (\log n)$ steps of the visit the queue grows to a size at least
$\beta_\epsilon \log n$. We provide more details of our techniques in
Subsection~\ref{ref.sec.tech} below. Finally, we highlight the sharp result
given by the theorem on the $\SWGm(n,c/n)$ model for the case $c = 1$:
similarly to the regular \SWGreg model, each node here has about one bridge
edge in average, and the obtained critical value for the contagion probability
turns out to be $\sqrt{2}-1$. An analysis of the critical value for
the \SWGreg model is given by the next two results, while a detailed comparison of the two
models is provided after Theorem~\ref{th:reg.upper} below.


\begin{theorem}[\SIR on the  \SWGreg model]\label{thm:main_matching-old}
Let $V$ be a set of $n$ vertices, $I_0 \subseteq V$, and $p > 0$ be a contagion probability. Sample a graph $G
= (V,E)$ from the \SWGreg distribution, and run the Reed-Frost SIR process on
$G$ with contagion probability $p$ and with the vertices in $I_0$ infectious at
time $0$. Then:

\begin{enumerate}
\item if $p>1/2+\varepsilon$, then with probability $\Omega_\varepsilon(1)$,
the \SIR \ process infects $\Omega_\varepsilon(n)$ nodes within time
$\bigO(n)$;
\item if $p<1/2-\varepsilon$, then, w.h.p., the \SIR \ process stops within
$\bigO_\varepsilon(\log n)$ rounds and the total number of infectious nodes is
$\bigO_\varepsilon(|I_0|\log n)$.
\end{enumerate}
\end{theorem}

In the above theorem, the first statement holds with constant probability over
the randomness of the generation of $G$ and the randomness of the contagion
process. 

The second statement holds with probability $1$ over the randomness of $G$ and
\emph{with high probability} over the randomness of the contagion process, and
it is a special case of the following more general result of ours.

\begin{theorem}[\SIR on bounded-degree graphs] 
\label{th:reg.upper-old}
Let $G=(V,E)$ be a graph of maximum degree $d$, $\varepsilon >0$ be an
arbitrary positive number, $p < (1-\varepsilon)/(d-1)$ be a contagion
probability, $I_0$ be a subset of $V$. Consider the Reed-Frost \SIR\
process on $G$ with initial set $I_0$ and contagion probability $p$.  Then,
w.h.p.,  the \SIR\ process stops within $\bigO_\varepsilon(\log n)$ steps and
infects $\bigO_\varepsilon ( |I_0| \log n)$ nodes.
\end{theorem}

\paragraph*{Consequences of our results.}
Because of a mix of local and random edges, epidemic spreading in the above
models proceeds as a sequence of outbreaks, a process that is made explicit in
our rigorous analysis, where we see the emergence of two qualitative
phenomena that are present in real-world epidemic spreading. 

One is that the presence of long-distance random connections has a stronger
effect on epidemic spreading than local connections, motivating lockdown
measures that shut down long-distance connections.  This can be seen,
quantitatively, in the fact that the critical probability in a cycle is $p =
1$, corresponding to a critical $r_0$ equal to 2. On the other hand, the
presence of random matching edges or random $\mathcal{G}_{n,c/n}$ edges in the
setting $c = 1$ defines networks in which the critical $r_0$ is, respectively,
$1.5$ and $3\cdot (\sqrt 2 -1) \approx 1.24$, meaning that notably fewer local
infections can lead to large-scale contagion on a global scale.

The other phenomenon is that  the irregular networks of the $\SWGm(n,c/n)$
model in the case $c=1$ show a significantly lower critical probability, i.e.
$\sqrt 2 -1 \approx .41$, than the  critical value $.5$ of the nearly regular networks of
the \SWGreg model, though they have the same number of edges (up to lower order
terms) and very similar distributions. As a further evidence of this
phenomenon, we remark the scenario yielded by the random irregular networks
sampled from the $\SWGm(n,c/n)$ distribution with $c$ even smaller than $1$:
for instance, the setting $c = .7$, though yielding a much sparser topology
than the \SWGreg networks, has a critical probability which is still smaller
than $.5$. Moreover, this significant difference between the $\SWGm(n,c/n)$
model and the regular $\SWGm$ one holds even for more dense regimes. In detail,
Theorem~\ref{th:reg.upper} implies that the  almost-regular version of $\SWGm$
in which $c$ independent random matchings are added to the ring of $n$ nodes
has a critical probability at least $1/(c+1)$. Then, simple calculus shows that
the critical probability given by Theorem~\ref{thm:gen_overthershold} for the
$\SWGm(n,c/n)$ model is smaller than $1/(c+1)$, for any choice  of the
density parameter $c$.

The most significant difference between the two distributions above  is the
presence of a small number of high-degree vertices in $\SWGm(n,c/n)$,
suggesting that even a small number of ``super-spreader'' nodes can have major
global consequences.


\paragraph*{Extensions of our results.}
Natural generalizations of the setting considered in this work include models in which i) the interval of time
during which a node is infectious (i.e., the \emph{activity period}) follows some (possibly node-dependent) distribution and/or ii) once infected, a node only becomes infectious after
an \emph{incubation} period, whose duration again follows some distribution.
While the introduction of activity periods following general distributions may considerably complicate the analysis, our approach rather straightforwardly extends to
two interesting cases, in which the incubation period of each node is a random variable (as long as incubation periods are independent) and/or the activity period of a node consists of $k$
consecutive units of time, with $k$ a fixed constant. 
This generalized model with random, node-dependent incubation periods corresponds to a discrete,
synchronous version of the $\mathrm{SEIR}$ model,\footnote{With respect to \SIR, for each node we have a fourth, \emph{Exposed} state, corresponding to the incubation period of a node.} which 
was recently considered as a model of the COVID-19 outbreak in Wuhan \cite{lin2020conceptual}.
These extensions are formalized and discussed in Section \ref{sec:further}.


\subsection{Our techniques}
\label{ref.sec.tech}


%\andy{Inserire una introduzione all'equivalenza IC $=$ BP process}

The starting point of our analysis is the   equivalence, proved by~\cite{KKT15} and mentioned above,  between  the Reed-Frost
SIR model and the bond percolation process.  We
will return to this equivalence, and state it more formally, in Subsection~\ref{ssec:equi}.

Given this equivalence, our goal is as follows: sample a graph
$G$ from $\SWGm(n,1/n)$ or \SWGreg,\footnote{For simplicity of exposition, in this informal description of
our techniques, we only consider the case $q = 1/n$ for the $\SWGm(n,q)$ model.} create the percolation graph $G_p$, by independently
deleting each edge of $G$ with probability $1-p$, and estimate the number of
vertices reachable from $I_0$ in $G_p$.

\noindent\textbf{Analyzing bond percolation.} A standard technique in bond percolation, applied for example to percolation in infinite trees and in random graphs, is to analyze the process of running a BFS in the percolation graph, delaying decisions about the percolation of edges from a node $w$ to unvisited vertices until the time $w$ is taken out of the BFS queue. In random graphs and infinite trees, the distribution of unvisited neighbors of $w$ in the percolation graph remains simple, even conditioned on previous history, and one can model the size of the BFS queue as a Galton-Watson process, thus reducing the percolation analysis to standard results about branching processes. Basically, if the number of vertices that we add at each step to the queue is less than one on average, the visit will reach on average a constant number of vertices and if it is more than one and the graph is infinite the visit will reach on average an infinite number of vertices. 

\noindent\textbf{Bond percolation in small-world graphs.} To study percolation in small-world graphs, it would be very difficult to analyze a BFS exploration of the percolation graph, because the distribution of unvisited neighbors of a vertex $w$ in the percolation graphs is highly dependent on the previous history of the BFS (in particular, it matters whether none, both, or one of the neighbors of $w$ along the cycle are already visited).

Instead, and this is one of the technical innovations of our work, we define a modified BFS visit whose process is more amenable to an analytical treatment. The main idea of our modified BFS is that in one step we do the following: after we pull a node $w$ from the queue,
we first look at the neighbors $x$ of $w$ that are reachable through bridge edges in the percolation graphs; then,
for each ``bridge neighbor'' $x$ of $w$, we visit the  ``local cluster'' of
$x$, that is, we explore the vertices reachable from $x$ along paths that only consist of edges of the cycle that are in the percolation graph; 
finally, we add to the queue all non-visited vertices in the local clusters of the bridge neighbors of $w$. These steps are exemplified in Fig. \ref{fig:local_cluster}.
%It is easy to see that the local cluster of each bridge neighbor has expected size $(1+p)/(1-p)$. 



The point of doing things this way is that if we delay decisions about the random choice of the bridge edges and the random choices of the percolation, then we have a good understanding both of the following two key random variables:

%\andy{Aggiungere una figura che rappresenti bene la situazione in expectation: un bridge che parte da $w$ ad $x$ ed intorno ad $x$ il local cluster e mettendo la dimensione attesa del LC e il numero atteso di $x$ ....}
\begin{figure}[htp]
    \centering
   \includegraphics[width=.9\textwidth]{./trunk-full/Images/process-queue.pdf}
    \caption{The figure shows an example in which the visit first proceeds from a node $w$ extracted from the queue to a new node $x$ over a bridge of the percolation graph and then reaches further nodes, starting from $x$ and proceeding along ring edges of the percolation graph. In terms of contagion, this corresponds to the virus first being transmitted from an infectious node $w$ to a susceptible one $x$ over a bridge edge and then propagating locally using ring edges. Note that in this case, i) we have a single bridge leaving $w$ (in general, there might be multiple ones) and  ii) the virus freely propagates locally from node $x$, infecting susceptible nodes $\ell_1,\ell_2,\ell_3$. The edges are directed in the direction of virus spread.}
    \label{fig:local_cluster}
\end{figure}


\begin{itemize}
    \item the number of bridge neighbors $x$ of $w$ along percolated bridge edges, which are, on average $pqn'$ if the graph comes from \SWG, $p$ is the percolation probability, and $n'$ is the number of unvisited vertices at that point in time;
    

 \item  the size of the ``local cluster'' of each such vertex $x$, that is of the vertices reachable from $x$ along percolated cycle edges, which has expectation 

\begin{equation}\label{eq:lc_intro}
    L = \frac{1+p}{1-p}\, .
\end{equation}

\end{itemize}

Intuitively, we would hope to argue that in our modified visit of a graph sampled from \SWG to which we apply percolation with activation probability $p$, the following happens in one step: we remove one node from the queue and we add on average 
\begin{equation}\label{eq:nn_intro}
    N = pqn' \cdot \frac{1+p}{1-p}
\end{equation}
new nodes. As long as $n' = n-o(n)$ we can approximate $n'$ with $n$, and when the number $n-n'$ of visited vertices is $\Omega(n)$ we are done. At this point, we would have modeled the size of the queue with a Galton-Watson process, and we would be done. The threshold behavior would occur at a $p$ such that $pqn \cdot (1+p)/(1-p) = 1$; a smaller value of $p$ would imply that at every step we remove one node and, on average, we add less than one node to the queue, leading the process to quickly die out; a larger value of $p$ would imply that at every step we remove one node and, on average, we add more than one node to the queue, leading the process to blow up until we reach $\Omega(n)$ vertices.


We are indeed able to prove this threshold behaviour, at least for $q = c/n$ for constant $c$, but we encounter a significant difficulty in making this idea rigorous:  if we proceed as described above, we would be double-counting vertices, because maybe the ``local cluster'' of a node added to the queue at a certain point collides with the local cluster of another node added at a later point. This is fine if we are trying to upper bound the number of reachable vertices, but it is a problem if we are trying to establish a lower bound.

To remedy this  difficulty, we truncate the exploration of each local cluster at a properly chosen constant size, and in our visit, we consider only unvisited neighbors $x$ of $w$ that are sufficiently far along the cycle from all previously visited vertices, so that there is always ``enough space'' to grow a truncated local cluster around $x$ without hitting already visited vertices. The truncation negligibly affects the average size of the local cluster, the restriction to a subset of unvisited vertices neglibly affects the distribution of unvisited neighbors, and the analysis carries through with the same parameters and without the ``collision of local clusters'' problems.

The truncation is such that our modified BFS does not discover all vertices reachable from $I_0$ in the percolation graph, but only a subset. This is sufficient, however, to prove lower bounds to the number of reachable vertices. Proving upper bounds is easier because, as mentioned, we can allow double-counting of reachable vertices.

\noindent\textbf{Further challenges in 3-regular small-world graphs.} An additional difficulty arises in the \SWGreg\ model, in which bridge edges form a random matching, since this model introduces additional dependencies on the past history, and we deal with this difficulty by disallowing an additional set of unvisited vertices $x$ to be reached in the visit. 

An important difference between the \SWGreg\ model and the \SWG\ model is that when we take a node $w$ out of the queue then there can be at most one unvisited neighbor $x$ of $w$ reachable through a bridge edge in the percolation graph. If such a neighbor $x$ exists, and it is not one of the disallowed unvisited vertices, we find, as before, the truncated local cluster of $x$ and add the nodes of the local cluster of $x$ to the queue, {\em except for $x$ itself}. The reason for discarding $x$ is that we have already observed the unique bridge neighbor of $x$ (namely, $w$), so, when we would take $x$ out of the queue later there would be no randomness left on which to apply deferred decision.

This means that, roughly speaking, in one step of our visit on \SWG\ with activation probability $p$, we take out one node from the queue and add on average a number of nodes described by \eqref{eq:nn_intro}, while in \SWGreg\ we take out one node and add on average
\begin{equation}\label{eq:3reg_intro}
    N' = p \cdot \frac{1+p}{1-p} - 1
\end{equation}
nodes. This is why, the \SWGreg\ model with $q=1/n$ and the \SWGreg\ model have notably different thresholds, even though they are superficially very similar.


\iffalse

Intuitively, if all newly observed bridge edges that are incident to $w$ connected $w$ to nodes that have
not been visited before, and if all corresponding local clusters only contained
nodes that have not yet been visited (which is a good approximation of what
happens as long as the number of visited nodes is $o(n)$), the number of
newly enqueued vertices upon processing of $w$ would be $p \cdot
(1+p)/(1-p)$ in expectation for the $\SWGm(n,1/n)$ model and $p \cdot ((1+p)/(1-p) - 1)$ for
\SWGreg\ model. The difference is that we have already observed at least one
bridge edge going into each bridge neighbor $x$ (the one by which we reached
$x$ and put it in the queue), and this condition negligibly changes the number
of remaining bridge edges if the bridge edges are sampled according to
$\SWGm(n,1/n)$, but it implies that there are no more bridges to observe out of
$w$ in the \SWGreg\ model (indeed, in the visit of graphs from \SWGreg\ model
we do not put in the queue the entire local cluster of each bridge neighbor
$x$, but the {\em local cluster minus the vertex $x$}).

If we study the number of edges in the queue of our modified BFS, at each
iteration it decreases by 1 when we dequeue an element, and then it increases,
on average, either by roughly $p \cdot (1+p)/(1-p)$ or by roughly $p \cdot
((1+p)/(1-p) - 1)$, as long as the total number of visited vertices is $o(n)$.
We can model the size of the queue as a Galton-Watson process (defined in
Section \ref{sec:GW} below), and we see that the critical value of $p$ is when
the expected number of nodes added to the queue in each iteration is one, that
is, $p \cdot (1+p)/(1-p) =1$ in the $\SWGm(n,1/n)$ model, which solves to $p =
\sqrt 2-1$, and  $p \cdot( (1+p)/(1-p) -1)=1$ in the \SWGreg model, which solves
to $p=1/2$. The coupling between the size of the queue and the Galton-Watson
process breaks down once $\Omega(n)$ vertices have been visited, but at that
point we have reached the conclusion that we are interested in.

To establish the coupling between our BFS-like visit and the Galton-Watson
process, we also have to ensure that, at every step, there is enough residual
randomness in the choice of the bridge edges and in the bond percolation
conditioned on what we have observed in previous step, an issue that is
particularly tricky in the random matching model.

To control the effect of conditioning on previous steps, our BFS-like visit
truncates the visit of the local cluster after a constant $L$ number of steps,
and maintains the invariant that the nodes in the queue are at distance $> 2L$
from one another along the cycle. This guarantees that the percolation events
that we observe for one node of the queue do not affect the events that we
observe later for another node of the queue. We put additional restrictions to
the vertices that we allow to be added to the queue to also reduce conditioning
effects on the bridge edges. 

\fi

In order to get bounds on contagion time, we study a visit as above only up to
the point in which there are order of $\log n$ nodes in the queue (if $I_0$ is
already of the order of $\log n$, this first phase of the analysis may be
skipped), and then we study a ``parallel'' visit in which we add at once all
the nodes reachable through a local cluster and one bridge edge from the nodes
currently in the queue, skipping those that would create problems with our
invariants. Here we are able to argue that, as long as the number of visited
vertices is $o(n)$, the number of nodes in the queue grows by a constant factor
in each iterations, and so we reach $\Omega(n)$ nodes in $\bigO(\log n)$ time. 

Currently, we are not able to analyze the parallel visit in the \SWGreg\ model,
because of the correlations between the edges, although we are able to analyse
the sequential search up to the point when it visits $\Omega(n)$ nodes. This is
why in our theorems we do not have logarithmic contagion time bounds for the
\SWGreg model.


\input{./trunk-full/Related.tex}






==> trunk-full/Related.tex <==
\subsection{Comparison to previous results}\label{subse:related}

As far as we know, our results are the first rigorous ones to establish
threshold phenomena in small-world graphs for the \SIR\ process  and for the
bond percolation process.

There has been some previous work on studying sufficient conditions for the
\SIR\ process  to reach a sublinear number of vertices. 

 
In~\cite{DGM06}, for a symmetric, connected graph $G = (V,E)$, Draief et al
prove a general lower bound on the critical point in the Independent Cascade
model in terms of spectral properties. Further versions of such bounds for
special cases have been subsequently derived in~\cite{LKAK16,LSV14}.
Specifically, if one lets $P$ be the matrix such that $P(u,v) = p(u,v)$ is the
probability of the edge $\{u,v\}$, and $P(u,v) = 0$ if $\{u,v\}\not\in E$, and
if one call $\lambda$ the largest eigenvalue of $P$, then $\lambda <
1-\epsilon$ implies that for a random start vertex $s$ we have that the
expected number of vertices to which $s$ spreads the infection is $o_\epsilon
(n)$.

In the special case in which all probabilities are the same, $P = p \cdot A$,
where $A$ is the adjacency matrix of $G$, and so the condition is asking for $p
< (1-\epsilon)/ \lambda_{\max{}} (A)$.

This condition is typically not tight, and it is never tight in the
``small-worlds'' graphs   we consider:

\begin{itemize}

\item In the  \SWGreg model, the largest eigenvalue of the adjacency matrix is
$3-o(1)$, but the critical probability is $1/2$ and not $1/3$;

\item In the $\SWGm(n,1/n)$ model of a cycle plus \Erdos\ edges, the largest
eigenvalue of the adjacency matrix is typically $\Omega(\sqrt{ \log n /
\log\log n})$, because we expect to see vertices of degree $\Omega(\log n /
\log\log n)$ and the largest eigenvalue of the adjacency matrix of a graph is
at least the square root of its maximal  degree. The spectral bound would only
tell us that the infection dies out if $p = \bigO(\sqrt{\log\log n / \log n})$,
which goes to zero with $n$.  A better way to use the spectral approach is to
model together the randomness of the small-world graph and the randomness of
the percolation; in this case we have matrix $P(u,v)$ such that $P(u,v)=p$ for
edges of the cycle and $P(u,v) = p/n$ for the other edges. This matrix has
largest eigenvalue $3p-o(1)$ and so the spectral method would give a
probability of $1/3$, while we are able to locate the threshold at $\sqrt 2
-1\approx .41$.
\end{itemize}

In any family of $d$-regular graphs, the largest eigenvalue of the adjacency
matrix is $d$, and so the spectral bound gives that the critical threshold is
at least $1/d$; our Theorem~\ref{th:reg.upper} shows the stronger bound that
the critical threshold is at least $1/(d-1)$.

We are not aware of previous rigorous results that provide sufficient
conditions for the Independent Cascade process to reach $\Omega(n)$ nodes
(either on average or with high probability) in general graphs, or for the
equivalent question of proving that the percolation graph of a given graph has
a connected component with $\Omega(n)$ vertices.


%\andy{Cambiare qui sotto: la discussione della nostra analisi e' ora sopra}

Our analysis, as discussed in the previous subsection, proceeds by analysing a
BFS-like visit of the percolation graph. This is also the way in which large
components in the percolation of infinite trees and in random graphs have been
studied before, but this idea requires considerable elaboration to work in our
setting, given the mix of fixed edges and random edges in the small-world
model, and the complicated dependencies on the past history that one has to
control in the analysis of the visit.





More generally, there is a very large body of work devoted to study of models of epidemic
spreading, as surveyed in~\cite{VespietAl15,Wang_2017}. In the following, we
review analytical studies of Independent Cascade on finite graphs.

In the Computer Science community, to the best of our knowledge, Kempe et al~\cite{KKT15}
were the first to investigate this model in an optimization perspective, in the context
of viral marketing and opinion diffusion. In particular, they introduced the \emph{Influence
Maximization} problem, where the goal is to find a subset of $k$ nodes of an underlying graph
to infect at time $t = 0$, so as to maximize the expected number of infected
nodes at the end of the Independent Cascade process. They prove this is an
$NP$-hard problem and show a polynomial time   algorithm achieving  constant
approximation.  Further approximation results on  a version of \emph{Influence
Maximization} in which the infection time is considered can be found
in~\cite{CWZ12,LGD12}.

A fundamental and rigorous study of bond percolation in random graphs has been proposed by Bollob\'as et al in~\cite{Bollo07}. 
They establish a coupling
between the bond percolation process and a suitably defined branching process.
In the   general class of inhomogenous \Erdos\ random graphs, calling $Q = \{
q_{u,v}\}$   the edge-probability matrix,  they derived the critical point
(threshold) of the phase transition and  the size of the giant component above
the transition. The  class  of inhomogeneous random graphs to which their
analysis applies includes  generative models that have been studied in the
complex network literature. For instance, a version of the Dubin's
model~\cite{Durrett1990ATT} can be expressed in this way, and so can the
\emph{mean-field scale-free model}~\cite{Bollobs2004TheDO}, which is, in turn,
related to the   Barabási–Albert model~\cite{Barab509}, having the same
individual edge probabilities, but with edges present independently. Finally,
we observe that the popular CHKNS model introduced by  Callaway et
al~\cite{CDHKNS01} can be analyzed using an edge-independent version of this
model. Indeed, they consider a random graph-formation process where, after
adding each node,   a Poisson  number of edges is added to the graph, again
choosing the endpoints of these edges uniformly at random.  For all such
important classes of random graph models, they show tight bounds for the
critical points and the relative size of the giant component beyond the phase
transition.

In our setting, if we sample a graph from $\SWGm(n,q)$ and then consider the
percolation graph $G_p$, the distribution of $G_p$ is that of an inhomogenous
\Erdos\ graph in which the cycle edges have probability $p$ and the remaining
edges have probability $pq$ (the \SWGreg model, however, cannot be expressed as
an inhomogenous \Erdos\ graph).

Unfortunately, if we try to apply the results of~\cite{Bollo07} to the
inhomogenous random graph equivalent to percolation with parameter $p$ in the
$\SWGm(n,q)$ model, we do not obtain tractable conditions on the critical
value $p$ for which the corresponding graph has a large connected component of
small diameter, which is the kind of result that we are interested in proving.

The \SIR process on the class of $1$-dimensional small-world networks (that is,
graphs obtained as the union of a cycle and of randomly chosen edges) has been
studied in~\cite{MCN00}: using numerical approximations on the moment
generating function, non-rigorous bounds on the critical threshold    have been
derived while analytical results are given neither  for the expected size of
the number of infected nodes above the transition phase of the SIR process nor
for the infection time.  Further non-rigorous results on the critical points of
several classes of complex networks have been derived in~\cite{LRSV14,LKAK16}
(for good surveys see~\cite{VespietAl15,Wang_2017}).


\subsection{Roadmap}

The rest of this paper is organized as follows. In Section~\ref{sec:prely}, we
provide  some key notions and preliminary results used throughout the paper. In Section~\ref{sec:wup}, we
describe our general approach, based on a suitable visiting process over the
percolation graph induced by the \SIR process: as a warm-up intended to highlight a few
key ingredients, we begin by deriving a lower bound on the final number of recovered nodes,
in the case of the \SIR process with the \SWG  model defining the underlying topology, for a 
single initiator, when infection probability is above the threshold. To begin, we focus on the
extent of the epidemic spreading, without considering the spreading time, for the sake of
presentation..
Section~\ref{sec:regularcase} provides the analysis of the \SIR process on the
\SWGreg model that proves Claim~$1$ of Theorem~\ref{thm:main_matching}.
Section~\ref{sec:boot} goes back to the  setting considered in
Section~\ref{sec:wup}, this time also addressing spreading time and proving (the stronger) Claims~$1$
and~$2$ of Theorem~\ref{thm:gen_overthershold}. The analysis of the \SIR
process in the  \SWG model below the threshold, which proves Claim~$3$ of
Theorem~\ref{thm:gen_overthershold}, is given in Section~\ref{sec:belo},
while the general result below the threshold  for regular graphs stated in
Theorem~\ref{th:reg.upper} is given in Section~\ref{sec:reg-gen}. In Section \ref{sec:further}, we 
show how our analysis generalizes to extensions of our model in which infected nodes
experience a (random) incubation period before becoming infected and/or they are infectious
for an activity period of fixed duration. Finally, the
mathematical tools and the proofs of some technical lemmas are given in the
Appendix. 



==> trunk-full/proofs_idea_fra.tex <==
\section{Proofs Ideas  } \label{sec:Proof Ideas}


FRANCESCO

\andy{Extend the informal description given in the old intro:
it would be nice to state some major technical lemmas and BFS algo}

\fra{Added the informal description with only minor changes to keep it
consistent with the new structure.}

\fra{Adding further details (technical lemmas, BFS pseudocode,...) with the
necessary definitions might make this section too long for the conference
version. May be we can add pointers to the appendix instead.}


\andy{Francesco, ora abbiamo molto piu spazio per la descrizione delle prove: vedi tu cosa aggiungere. Magari mettere almeno uno degli pseudocde delle visite con il concetto piu semplice di nodi free, inoltre alcuni statement tecnici forse possono essere messi in modo non rigorosi senza richiedere definizioni precise.... }

A standard technique in bond percolation, applied for example to percolation in
infinite trees and in random graphs, is to analyze the process of running a BFS
in the percolation graph, delaying decisions about the percolation of edges
from a node $w$ to unvisited vertices until the time $w$ is taken out of the
BFS queue. In random graphs and infinite trees, the distribution of unvisited
neighbors of $w$ in the percolation graph remains simple, even conditioned on
previous history, and one can model the size of the BFS queue as a
Galton-Watson process (see Definition \ref{def:GW}), thus reducing the percolation analysis to standard results about branching processes. Basically, if the number of vertices that we add at each step to the queue is less than one on average, the visit will reach on average a constant number of vertices and if it is more than one and the graph is infinite the visit will reach on average an infinite number of
vertices. 

\subsection{ Bond percolation in small-world graphs - Sketch of proof of
Theorem~\ref{thm:gen_overthershold}.} 

To study percolation in small-world
graphs, it would be very difficult to analyze a BFS exploration of the
percolation graph, because the distribution of unvisited neighbors of a vertex
$w$ in the percolation graphs is highly dependent on the previous history of
the BFS (in particular, it matters whether none, both, or one of the neighbors
of $w$ along the cycle are already visited).

Instead, and this is one of the technical innovations of our work, we define a
modified BFS visit whose process is more amenable to an analytical treatment.
The main idea of our modified BFS is that in one step we do the following:
after we pull a node $w$ from the queue, we first look at the neighbors $x$ of
$w$ that are reachable through bridge edges in the percolation graphs; then,
for each ``bridge neighbor'' $x$ of $w$, we visit the  ``local cluster'' of
$x$, that is, we explore the vertices reachable from $x$ along paths that only
consist of edges of the cycle that are in the percolation graph; finally, we
add to the queue all non-visited vertices in the local clusters of the bridge
neighbors of $w$. These steps are exemplified in Fig.~\ref{fig:local_cluster}.

The point of doing things this way is that if we delay decisions about the
random choice of the bridge edges and the random choices of the percolation,
then we have a good understanding both of the following two key random
variables:

\begin{figure}
\centering
\includegraphics[width=.9\textwidth]{./trunk-full/Images/process-queue.pdf}
\caption{The figure shows an example in which the visit first proceeds from a
node $w$ extracted from the queue to a new node $x$ over a bridge of the
percolation graph and then reaches further nodes, starting from $x$ and
proceeding along ring edges of the percolation graph. In terms of contagion,
this corresponds to the virus first being transmitted from an infectious node
$w$ to a susceptible one $x$ over a bridge edge and then propagating locally
using ring edges. Note that in this case, i) we have a single bridge leaving
$w$ (in general, there might be multiple ones) and  ii) the virus freely
propagates locally from node $x$, infecting susceptible nodes
$\ell_1,\ell_2,\ell_3$. The edges are directed in the direction of virus
spread.}
\label{fig:local_cluster}
\end{figure}


\begin{itemize}

\item the number of bridge neighbors $x$ of $w$ along percolated bridge edges,
which are, on average $pqn'$ if the graph comes from \SWG, $p$ is the
percolation probability, and $n'$ is the number of unvisited vertices at that
point in time;

\item the size of the ``local cluster'' of each such vertex $x$, that is of the
vertices reachable from $x$ along percolated cycle edges, which has expectation 

\begin{equation}\label{eq:lc_intro}
    L = \frac{1+p}{1-p}\, .
\end{equation}

\end{itemize}

Intuitively, we would hope to argue that in our modified visit of a graph
sampled from \SWG to which we apply percolation with activation probability
$p$, the following happens in one step: we remove one node from the queue and
we add on average 
\begin{equation}\label{eq:nn_intro}
    N = pqn' \cdot \frac{1+p}{1-p}
\end{equation}
new nodes. As long as $n' = n-o(n)$ we can approximate $n'$ with $n$, and when
the number $n-n'$ of visited vertices is $\Omega(n)$ we are done. At this
point, we would have modeled the size of the queue with a Galton-Watson
process, and we would be done. The threshold behavior would occur at a $p$ such
that $pqn \cdot (1+p)/(1-p) = 1$; a smaller value of $p$ would imply that at
every step we remove one node and, on average, we add less than one node to the
queue, leading the process to quickly die out; a larger value of $p$ would
imply that at every step we remove one node and, on average, we add more than
one node to the queue, leading the process to blow up until we reach
$\Omega(n)$ vertices.

We are indeed able to prove this threshold behaviour, at least for $q = c/n$
for constant $c$, but we encounter a significant difficulty in making this idea
rigorous:  if we proceed as described above, we would be double-counting
vertices, because maybe the ``local cluster'' of a node added to the queue at a
certain point collides with the local cluster of another node added at a later
point. This is fine if we are trying to upper bound the number of reachable
vertices, but it is a problem if we are trying to establish a lower bound.

To remedy this  difficulty, we truncate the exploration of each local cluster
at a properly chosen constant size, and in our visit, we consider only
unvisited neighbors $x$ of $w$ that are sufficiently far along the cycle from
all previously visited vertices, so that there is always ``enough space'' to
grow a truncated local cluster around $x$ without hitting already visited
vertices. 

\andy{Inserire qui la definizione formale di free node (caso base): mi sembra che non servano altre definizioni }


The truncation negligibly affects the average size of the local
cluster, the restriction to a subset of unvisited vertices neglibly affects the
distribution of unvisited neighbors, and the analysis carries through with the
same parameters and without the ``collision of local clusters'' problems.

\andy{Inserire qui la MODIFIED BFS (caso Base)}

The truncation is such that our modified BFS does not discover all vertices
reachable from $I_0$ in the percolation graph, but only a subset. This is
sufficient, however, to prove lower bounds to the number of reachable vertices.
Proving upper bounds is easier because, as mentioned, we can allow
double-counting of reachable vertices.

\fra{We need to replce ``Contagion time'' in the paragraph below with something
appropriate (e.g., ``distance from the source'')}

\andy{Si, parliamo sempre di distanze ...}


\andy{Inserire qui il main Lemma tecnico dell'ex warm-up e modificare
qui sotto }

In order to get bounds on \textcolor{red}{contagion time}, we study a visit as
above only up to the point in which there are order of $\log n$ nodes in the
queue (if $I_0$ is already of the order of $\log n$, this first phase of the
analysis may be skipped), and then we study a ``parallel'' visit in which we
add at once all the nodes reachable through a local cluster and one bridge edge
from the nodes currently in the queue, skipping those that would create
problems with our invariants. 

\andy{mettere un pointer alla BFS parallela ed al lemma formale: magari 
segnalare che gestiamo le correlazioni in modo tale che la crescita esponenziale
dei livelli e' provata whp... }




Here we are able to argue that, as long as the
number of visited vertices is $o(n)$, the number of nodes in the queue grows by
a constant factor in each iterations, and so we reach $\Omega(n)$ nodes in
$\bigO(\log n)$ time. 



\subsection{Further challenges in 3-regular small-world graphs: Sketch of
proof of Theorem~\ref{thm:main_matching}} An additional difficulty arises in
the \SWGreg\ model, in which bridge edges form a random matching, since this
model introduces additional dependencies on the past history, and we deal with
this difficulty by disallowing an additional set of unvisited vertices $x$ to
be reached in the visit. 

An important difference between the \SWGreg\ model and the \SWG\ model is that
when we take a node $w$ out of the queue then there can be at most one
unvisited neighbor $x$ of $w$ reachable through a bridge edge in the
percolation graph. If such a neighbor $x$ exists, and it is not one of the
disallowed unvisited vertices, we find, as before, the truncated local cluster
of $x$ and add the nodes of the local cluster of $x$ to the queue, {\em except
for $x$ itself}. The reason for discarding $x$ is that we have already observed
the unique bridge neighbor of $x$ (namely, $w$), so, when we would take $x$ out
of the queue later there would be no randomness left on which to apply deferred
decision.

This means that, roughly speaking, in one step of our visit on \SWG\ with
activation probability $p$, we take out one node from the queue and add on
average a number of nodes described by \eqref{eq:nn_intro}, while in \SWGreg\
we take out one node and add on average
\begin{equation}\label{eq:3reg_intro}
    N' = p \cdot \frac{1+p}{1-p} - 1
\end{equation}
nodes. This is why, the \SWGreg\ model with $q=1/n$ and the \SWGreg\ model have
notably different thresholds, even though they are superficially very similar.

Currently, we are not able to analyze the parallel visit in the \SWGreg\ model,
because of the correlations between the edges, although we are able to analyse
the sequential search up to the point when it visits $\Omega(n)$ nodes. This is
why in our theorems we do not have logarithmic contagion time bounds for the
\SWGreg model.




==> trunk-full/proofs_idea_part_1.tex <==
\section{Technical Proofs: An Overview} \label{sec:Proof Ideas}


A standard technique in bond percolation, applied for example to percolation in
infinite trees and in random graphs, is to analyze the process of running a BFS
in the percolation graph, delaying decisions about the percolation of edges
from a node $w$ to unvisited vertices until the time $w$ is taken out of the
BFS queue. In random graphs and infinite trees, the distribution of unvisited
neighbors of $w$ in the percolation graph remains simple, even conditioned on
previous history, and one can model the size of the BFS queue as a
Galton-Watson process (see Definition \ref{def:GW}), thus reducing the percolation analysis to standard results about branching processes. Basically, if the number of vertices that we add at each step to the queue is less than one on average, the visit will reach on average a constant number of vertices and if it is more than one and the graph is infinite the visit will reach on average an infinite number of
vertices. 

\subsection{ Proof of
Theorem~\ref{thm:gen_overthershold}: Bond percolation in the \SWG model} 

To study percolation in the small-world
 model \SWG, it would be very difficult to analyze a BFS exploration of the
percolation graph, because the distribution of unvisited neighbors of a vertex
$w$ in the percolation graphs is highly dependent on the previous history of
the BFS (in particular, it matters whether none, both, or one of the neighbors
of $w$ along the cycle are already visited).

Instead, and this is one of the technical innovations of our work, we define a
modified BFS visit whose process is more amenable to an analytical treatment.
The main idea of our modified BFS is that in one step we do the following:
after we pull a node $w$ from the queue, we first look at the neighbors $x$ of
$w$ that are reachable through bridge edges in the percolation graphs; then,
for each ``bridge neighbor'' $x$ of $w$, we visit the  ``local cluster'' of
$x$, that is, we explore the vertices reachable from $x$ along paths that only
consist of edges of the cycle that are in the percolation graph; finally, we
add to the queue all non-visited vertices in the local clusters of the bridge
neighbors of $w$. These steps are exemplified in Fig.~\ref{fig:local_cluster}.

The point of doing things this way is that if we delay decisions about the
random choice of the bridge edges and the random choices of the percolation,
then we have a good understanding both of the following two key random
variables:

\begin{figure}
\centering
\includegraphics[width=.9\textwidth]{./trunk-full/Images/process-queue.pdf}
\caption{The figure shows an example in which the visit first proceeds from a
node $w$ extracted from the queue to a new node $x$ over a bridge of the
percolation graph and then reaches further nodes, starting from $x$ and
proceeding along ring edges of the percolation graph. In terms of contagion,
this corresponds to the virus first being transmitted from an infectious node
$w$ to a susceptible one $x$ over a bridge edge and then propagating locally
using ring edges. Note that in this case, i) we have a single bridge leaving
$w$ (in general, there might be multiple ones) and  ii) the virus freely
propagates locally from node $x$, infecting susceptible nodes
$\ell_1,\ell_2,\ell_3$. The edges are directed in the direction of virus
spread.}
\label{fig:local_cluster}
\end{figure}


\begin{itemize}

\item the number of bridge neighbors $x$ of $w$ along percolated bridge edges,
which are, on average $pqn'$ if the graph comes from \SWG, $p$ is the
percolation probability, and $n'$ is the number of unvisited vertices at that
point in time;

\item the size of the ``local cluster'' of each such vertex $x$, that is of the
vertices reachable from $x$ along percolated cycle edges, which has expectation 

\begin{equation}\label{eq:lc_intro}
    L = \frac{1+p}{1-p}\, .
\end{equation}

\end{itemize}

Intuitively, we would hope to argue that in our modified visit of a graph
sampled from \SWG to which we apply percolation with   probability
$p$, the following happens in one step: we remove one node from the queue and
we add on average 
\begin{equation}\label{eq:nn_intro-new}
    N = pqn' \cdot \frac{1+p}{1-p}
\end{equation}
new nodes. As long as $n' = n-o(n)$ we can approximate $n'$ with $n$, and when
the number $n-n'$ of visited vertices is $\Omega(n)$ we are done. At this
point, we would have modeled the size of the queue with a Galton-Watson
process, and we would be done. The threshold behavior would occur at a $p$ such
that $pqn \cdot (1+p)/(1-p) = 1$; a smaller value of $p$ would imply that at
every step we remove one node and, on average, we add less than one node to the
queue, leading the process to quickly die out; a larger value of $p$ would
imply that at every step we remove one node and, on average, we add more than
one node to the queue, leading the process to blow up until we reach
$\Omega(n)$ vertices.

We are indeed able to prove this threshold behaviour, at least for $q = c/n$
for constant $c$, but we encounter a significant difficulty in making this idea
rigorous:  if we proceed as described above, we would be double-counting
vertices, because maybe the ``local cluster'' of a node added to the queue at a
certain point collides with the local cluster of another node added at a later
point. This is fine if we are trying to upper bound the number of reachable
vertices, but it is a problem if we are trying to establish a lower bound.

To remedy this  difficulty, we truncate the exploration of each local cluster
at a properly chosen constant size (we denote it as $\LC ^L$), and in our visit, we consider only
unvisited neighbors $x$ of $w$ that are sufficiently far along the cycle from
all previously visited vertices, so that there is always ``enough space'' to
grow a truncated local cluster around $x$ without hitting already visited
vertices. More in detail, we introduce the notion of ``\good node'', that is used
 in the algorithm and in its analysis.
 
 \begin{definition}[\good node]\label{def:free_node}
Let $G_{SW} = (V, E_1 \cup E_2)$ be a small-world graph and let $L \in
\mathbb{N}$. We say that a node $x \in V$ is  \good for a subset of nodes $X
\subseteq V$ if $x$ is at distance at least $L+1$ from any node in $X$ in the
subgraph $(V, E_1)$ induced by the edges of the ring.
\end{definition}


Thanks to the above definition, we can now formalize our modified BFS.

\begin{algorithm}[H]
\caption{Sequential \SIRimmtrunc}
\small{
\textbf{Input}: A small-world graph $G_{\text{SW}} = (V, E_{\text{SW}})$, the 
bond-percolation subgraph $H$, and a set of initiators $I_0 \subseteq V$.

    \begin{algorithmic}[1]
	\State $Q = I_0$
	\State $R = \emptyset$
	\While{$Q \neq \emptyset $}
	    \State $w = \dequeue(Q)$
	    \State $R = R \cup \{w\}$ 
 	            \For {each bridge neighbor $x$ of $w$ in $H$}
 	              \If {$x$ is \good for $R \cup Q$ in $G_{SW}$}
 	                  \For{each node $y$ in the $L$-truncated local cluster $\LC ^L (x)$} 
 	                       \State $\enqueue(y,Q)$
 	                  \EndFor
 	                
 	              \EndIf
 	            \EndFor
 	 \EndWhile
	\end{algorithmic}}
\label{alg:L-visit-intro}
\end{algorithm}


Tu sum-up, 
  the $L$-truncation negligibly affects the average size of the local
cluster, the restriction to a subset of unvisited vertices neglibly affects the
distribution of unvisited neighbors, and the analysis carries through with the
same parameters and without the ``collision of local clusters'' problems.

% As an overview  of our general approach, we consider the percolation graph $G_p$ of a graph sampled from the $\SWGm(n,q)$ model with parameters $p$ and $q =
%c/n$, where $c$ is any positive constant such that $p \cdot q = pc/n <
%1$\footnote{Notice that if $p \cdot q \geq 1$, the analysis is trivial and all
%nodes will be infected, w.h.p.}.

In more detail, thanks to the   arguments we described above, from \eqref{eq:lc_intro} and \eqref{eq:nn_intro-new}, we can  prove Claim 1 of Theorem \ref{thm:gen_overthershold}:   if 
  $p$ is above the critical threshold

\begin{equation}
    \frac{\sqrt{c^{2} + 6c +1}-c-1}{2c} \, ,
\end{equation}
then, with probability $\Omega(1)$, the connected components of
$G_p$ containing the initiator subset have overall size $\Omega(n)$. In terms of our BFS visit in Figure \ref{alg:L-visit-intro}, we in fact derive  the following result\footnote{We state the result for    the case   $|I_0|=1|$.}.

 




\begin{lemma}\label{le:L-visit}
Let $V$ be a set of $n$ nodes and let $s \in V$ be an \textit{initiator} node.
For every $\varepsilon >0$ and $c>0$, and for every   probability   $p$
such that
\[
\frac{\sqrt{c^{2} + 6c +1}-c-1}{2c} + \varepsilon \leq p \leq  1 \, , 
\]
there are positive parameters $L,k,\varepsilon'$, and $\gamma$, that depend
only on $c$ and $\varepsilon$, such that the following holds.  Sample a graph
$G = (V,E)$ according to the $\SWGm(n, c/n)$ distribution and let $G_p$ be the
percolation graph of $G$ with parameter $p$.  Run the $L$-visit procedure in
Figure~\ref{alg:L-visit-intro} on input $(G,G_p,s)$: if $n$ is sufficiently large,
for every sufficiently large $t$, at the end of the $t$-th iteration of the
while loop it holds that 
\[
\Prc{|R \cup Q| \geq n/k \mbox{ \emph{OR} } |Q| \geq \varepsilon' t} \geq
\gamma \, , 
\]
where the probability is over both the randomness of the choice of $G$ from
$\SWGm(n, c/n)$ and over the choice of the percolation graph $G_p$.
\end{lemma}

We remark that the  truncation is such that our modified BFS does not discover all vertices
reachable from $I_0$ in the percolation graph, but only a subset. This is
sufficient, however, to prove lower bounds to the number of reachable vertices.
Proving upper bounds is easier because, as mentioned, we can allow
double-counting of reachable vertices.






\paragraph{Proof of Claim 2 of Theorem \ref{thm:gen_overthershold}: Bounding the number of hops.}
In order to get bounds on the size of the BFS levels, we study a visit as
above only up to the point in which there are order of $\log n$ nodes in the
queue (if $I_0$ is already of the order of $\log n$, this first phase of the
analysis may be skipped), and then we study a ``\emph{parallel}'' visit in which we
add at once all the nodes reachable through an $L$-trunkated local cluster (thus having constant diameter) and through one bridge 
from the nodes currently in the queue, skipping those that would create
problems with our invariants: to this aim, we need a stronger version of the notion
of \good node (see Definition \ref{def:good_nodes_par} in Appendix \ref{ssec:expgrowth}.)


Here we are able to argue that, as long as the
number of visited vertices is $o(n)$, the number of nodes in the queue grows by
a constant factor in each iterations, and so we reach $\Omega(n)$ nodes in
$\bigO(\log n)$ number of iterations that corresponds to $\bigO(\log n)$ distance from the source subset in the percolation subgraph $G_p$. 

A technical issue that we need to address in the analysis of our parallel visit  is that the random variables that count the contribution of each $L$-truncated local cluster,  added during one iteration of the visit, are not mutually independent.
To prove concentration results for 
this exponential growth, we thus need to  show that such a mutual correlation satisfies  a certain \emph{local} property and then apply suitable bounds for 
partly dependent random variables~\cite{Svante04} (see
Theorem~\ref{thm:svante} in Appendix~\ref{app:maths})). 

All details of this part can be found in   Appendix  \ref{ssec:expgrowth}.






\subsection{Further challenges in regular small-world graphs: Proofs of Theorems~\ref{thm:main_matching} and } 

An additional difficulty arises in
the \SWGreg\ model, in which bridge edges form a random matching, since this
model introduces additional dependencies on the past history, and we deal with
this difficulty by disallowing an additional set of unvisited vertices $x$ to
be reached in the visit. 

An important difference between the \SWGreg\ model and the \SWG\ model is that
when we take a node $w$ out of the queue then there can be at most one
unvisited neighbor $x$ of $w$ reachable through a bridge edge in the
percolation graph. If such a neighbor $x$ exists, and it is not one of the
disallowed unvisited vertices, we find, as before, the truncated local cluster
of $x$ and add the nodes of the local cluster of $x$ to the queue, {\em except
for $x$ itself}. The reason for discarding $x$ is that we have already observed
the unique bridge neighbor of $x$ (namely, $w$), so, when we would take $x$ out
of the queue later there would be no randomness left on which to apply deferred
decision.

This means that, roughly speaking, in one step of our visit on \SWG\ with
activation probability $p$, we take out one node from the queue and add on
average a number of nodes described by \eqref{eq:nn_intro-new}, while in \SWGreg\
we take out one node and add on average
\begin{equation}\label{eq:3reg_intro}
    N' = p \cdot \frac{1+p}{1-p} - 1
\end{equation}
nodes. This is why, the \SWGreg\ model with $q=1/n$ and the \SWGreg\ model have
notably different thresholds, even though they are superficially very similar.

The above argument allows us to prove Claims 1 and 2 of Theorem \ref{thm:main_matching}.

Currently, we are not able to analyze the parallel visit in the \SWGreg\ model,
because of the correlations between the edges, although we are able to analyse
the sequential search up to the point when it visits $\Omega(n)$ nodes. This is
why in our theorems we do not have an exponential growth of the BFS levels for the
\SWGreg model.

As for Claim 3 of Theorem \ref{thm:main_matching}, as remarked in Section \ref{sec:ourresults}, this is a direct consequence of the more general bounds
given by our  Theorem \ref{th:reg.upper}:
given any graph  $G=(V,E)$     of maximum degree $d$ and a percolation probability  $p < (1-\varepsilon)/(d-1)$, w.h.p.,   the number of nodes connected to any given source subset $I_0$ in $G_p$ is  $\bigO_\varepsilon (|I_0| \log n)$.

The proof of the above result again relies on a suitable BFS visit of the percolation subgraph $G_p$ which is similar to that in Figure \ref{alg:L-visit-intro} we used in the previous subsection. Informally, since the input  graph has maximum degree $d$, we are able to 
show that, if the procedure runs for $t$ iterations of the while loop, then it visits $t$ nodes:  very importantly, it has observed at most $t\cdot
(d-1)+1$ Bernoulli random variables with parameter $p = (1-\varepsilon)/(d-1)$ (namely the percolation of each visited edge)
and we found that at least $t$ of them were $1$. By Chernoff bounds, this
happens with probability $\exp(-\varepsilon^2 t/3)$.
  
  
  

\andy{Migliorare il  paragrafo qui sopra per la prova del Thm del lower bound 
su grafi regolari generici }



